LivePortrait: Efficient Portrait Animation with Stitching and Retargeting Control

Portrait Animation aims to synthesize a lifelike video from a single source image, using it as an appearance reference, with motion (i.e., facial expressions and head pose) derived from a driving video, audio, text, or generation. Instead of following mainstream diffusion-based methods, we explore and extend the potential of the implicit-keypoint-based framework, which effectively balances computational efficiency and controllability. Building upon this, we develop a video-driven portrait animation framework named LivePortrait with a focus on better generalization, controllability, and efficiency for practical usage. To enhance the generation quality and generalization ability, we scale up the training data to about 69 million high-quality frames, adopt a mixed image-video training strategy, upgrade the network architecture, and design better motion transformation and optimization objectives. Additionally, we discover that compact implicit keypoints can effectively represent a kind of blendshapes and meticulously propose a stitching and two retargeting modules, which utilize a small MLP with negligible computational overhead, to enhance the controllability. Experimental results demonstrate the efficacy of our framework even compared to diffusion-based methods. The generation speed remarkably reaches 12.8ms on an RTX 4090 GPU with PyTorch. The inference code and models are available at https://github.com/KwaiVGI/LivePortrait

==> affilation_ref.tex <==
%
%% just author list reference
% \author{Jianzhu Guo$^{1,2}$ \quad Xiangyu Zhu$^{1,2}$ \quad Chenxu Zhao$^{3}$ \quad Dong Cao$^{1,2}$ \quad Zhen Lei$^{1,2}$\thanks{Corresponding author} \quad Stan Z. Li$^{1,4,5}$\\
% %CBSR, NLPR, CASIA\\
% \small  $^{1}$ CBSR \& NLPR, Institute of Automation, Chinese Academy of Sciences, Beijing, China\\
% \small  $^{2}$School of Artificial Intelligence, University of Chinese Academy of Sciences, Beijing 100049, China\\
% \small	$^{3}$Mininglamp Academy of Sciences, Mininglamp Technology\\
% \small	$^{4}$Faculty of Information Technology, Macau University of Science and Technology, Macau SAR, China\\
% \small	$^{5}$School of Engineering, Westlake University, Hangzhou, China\\
% {\tt\small \{jianzhu.guo, xiangyu.zhu, dong.cao, zlei, szli\}@nlpr.ia.ac.cn, zhaochenxu@mininglamp.com} %, boahancock29@126.com
% % For a paper whose authors are all at the same institution,
% % omit the following lines up until the closing ``}''.
% % Additional authors and addresses can be added with ``\and'',
% % just like the second author.
% % To save space, use either the email address or home page, not both
% }
%

